MLPerf Mobile Inference Benchmark

This paper presents the first industry-standard open-source machine learning (ML) benchmark to allow perfor mance and accuracy evaluation of mobile devices with different AI chips and software stacks. The benchmark draws from the expertise of leading mobile-SoC vendors, ML-framework providers, and model producers. It comprises a suite of models that operate with standard data sets, quality metrics and run rules. We describe the design and implementation of this domain-specific ML benchmark. The current benchmark version comes as a mobile app for different computer vision and natural language processing tasks. The benchmark also supports non-smartphone devices, such as laptops and mobile PCs. Benchmark results from the first two rounds reveal the overwhelming complexity of the underlying mobile ML system stack, emphasizing the need for transparency in mobile ML performance analysis. The results also show that the strides being made all through the ML stack improve performance. Within six months, offline throughput improved by 3x, while latency reduced by as much as 12x. ML is an evolving field with changing use cases, models, data sets and quality targets. MLPerf Mobile will evolve and serve as an open-source community framework to guide research and innovation for mobile AI.

==> table/high-order_system_characteristics.tex <==
& ImageNet & ImageNet & COCO & ADE20K & SQuAD \\\hline
& MobileNetEdge & MobileNetEdge & SSD - MobileNetv2 &\pbox{20cm}{DeeplabV3+ \\ MobileNetv2} & MobileBERT \\\hline
MediaTek & \pbox{20cm}{UINT8+\\NNAPI (neuron-ann)+\\APU} & N/A & \pbox{20cm}{UINT8+\\NNAPI (neuron-ann)+\\APU} & \pbox{20cm}{UINT8+\\NNAPI (neuron-ann)+\\APU} & \pbox{20cm}{FP16+\\TFLite Delegate+\\Mali-GPU} \\\hline
Samsung & \pbox{20cm}{INT8+\\ENN+\\NPU} & \pbox{20cm}{INT8+\\ENN+\\NPU} & \pbox{20cm}{INT8+\\ENN+\\(NPU,CPU)} & \pbox{20cm}{INT8+\\ENN+\\GPU} \\ \hline
Qualcomm & \pbox{20cm}{UINT8+\\SNPE+\\AIP}





==> tex/acknowledgements.tex <==
\section*{Acknowledgements}

\noindent The MLPerf Mobile team would like to acknowledge several individuals for their effort. In addition to the team that architected the benchmark, MLPerf Mobile is the work of many who also helped produce the first set of results.

\paragraph{Arm:}
 Ian Forsyth,
 James Hartley,
 Simon Holland,
 Ray Hwang,
 Ajay Joshi,
 Dennis Laudick,
 Colin Osborne,
 and Shultz Wang.

\paragraph{dviditi:}
 Anton Lokhmotov.

\paragraph{Google:}
 Bo Chen,
 Suyog Gupta,
 Andrew Howard,
 and Jaeyoun Kim.

\paragraph{Harvard University:}
 Yu-Shun Hsiao. 

\paragraph{Intel:}
 Thomas Baker,
 Srujana Gattupalli,
 and Maxim Shevtsov.

\paragraph{MediaTek:}
 Kyle Guan-Yu Chen,
 Allen Lu,
 Ulia Tseng,
 and Perry Wang.

\paragraph{MLCommons:}
 Relja Markovic.

\paragraph{Qualcomm:}
 Mohit Mundhra.

\paragraph{Samsung:}
Dongwoon Bai,
 Stefan Bahrenburg,
 Jihoon Bang,
 Long Bao,
 Yoni Ben-Harush,
 Yoojin Choi,
 Fangming He,
 Amit Knoll,
 Jaegon Kim,
 Jungwon Lee,
 Sukhwan Lim,
 Yoav Noor,
 Muez Reda,
 Hai Su,
 Zengzeng Sun,
 Shuangquan Wang,
 Maiyuran Wijay,
 Meng Yu,
 and George Zhou.

\paragraph{Xored:}
Ivan Osipov
and Daniil Efremo.

==> tex/consumer_benefit.tex <==
\section{Myriad Use Cases}
\label{Value}

% Measuring mobile-AI performance in a fair, reproducible, and useful manner is challenging but not intractable. The need for transparency owes to the massive hardware and software diversity, which often tightly coupled with the intricacies of deployment scenarios, developer options, OEM life cycles, and so on. 

% MLPerf Mobile focuses on transparency for consumers by packaging the submitted code into an app. Figure~\ref{fig:mlperfapp_startup} shows the MLPerf Mobile startup screen.  With a simple tap on the ``Go'' button, the app runs all benchmarks by default, following the prescribed run rules (Figure~\ref{fig:mlperfapp_go}), and displays the results. It reports both performance and accuracy for all benchmark tasks (Figure~\ref{fig:mlperfapp_run}) and permits the user to view the results for each one (Figure~\ref{fig:mlperfapp_results}). Furthermore, the configuration that generates the results is also transparent (Figure~\ref{fig:mlperfapp_config}). The application runs on Android, though future versions will likely support iOS as well.

While we highlight a few interesting observations, there are many other benchmark use cases in the wild.

%We briefly summarize how the benchmark benefits each group.

\textbf{Application developers} want to know what real-world performance may look like on a device. The benchmark provides insight into the software frameworks on the various ``phones'' (i.e., SoCs) for these application developers. More specifically, the benchmark can help them quickly identify the most optimal solution for a given platform. For application developers who deploy their products ``into the wild,'' the benchmark and the various machine-learning tasks offer a deep perspective on the end-user experience for an actual mobile AI application.  

\textbf{OEMs} want to standardize the performance assessment methodology across different mobile chipset offerings. SoC vendors employ the same tasks, models, data sets, metrics, and run rules, making the results comparable and reproducible. Given the hardware ecosystem's vast heterogeneity, the standardization that the benchmark provides is vital for progress. 

\textbf{Model designers} want to package new machine learning models into the mobile app so that organizations can then easily share and reproduce the results. The app, coupled with the LoadGen, allows model designers to test and evaluate the model’s performance on a real device rather than using operation counts and model size as heuristics to estimate performance. This feature closes the gap between model designers and hardware vendors---groups that have struggled to share information efficiently and effectively. 

%We have open-sourced the app to allow others to experiment with it~\cite{GitHub URL coming soon}.\textcolor{red}{??}

\textbf{Mobile users} wants to make informed purchasing decisions. Many users want to know whether upgrading their phone to the latest chipset will meaningfully improve their experience. To this end, they want public, accessible information about various devices---something MLPerf Mobile provides. In addition, some power users want to measure their device’s performance and share that information with performance-crowdsourcing platforms. Both are important reasons for having an easily reproducible mechanism for measuring mobile-AI performance.

\textbf{Researchers} often require reproducibility to push state-of-the-art technologies. As such, researchers can employ the mobile-app framework to test their methods and techniques for improving model performance, quality, or both. The framework is open-source and freely accessible to academia~\cite{MLCmobile-app}. The app can enable  researchers to integrate their ML optimizations and reproduce more recent results from the literature. 

\textbf{Technical analysts} rely on reproducibility and transparency to provide an ``apples-to-apples'' comparison to assess generational performance improvements. MLPerf Mobile makes it easy to reproduce vendor-claimed results and interpret them because it shows how the device achieves a particular performance number and how it is using the hardware accelerator. 

%% overview of the vendor data


% \begin{figure*}[t!]
%         \centering
%         \subfloat[Startup screen]{
%         \includegraphics[trim=00 0 00 0, clip, height=2.8in]{fig/mobile1.pdf}
%         \label{fig:mlperfapp_startup}
%         }
%         \hfill
%         \subfloat[Running the benchmarks]{\includegraphics[trim=00 0 0 0, clip,height=2.8in]{fig/mobile2.pdf}
%         \label{fig:mlperfapp_go}
%         }
%         \hfill
%         \subfloat[Reporting results]{\includegraphics[trim=00 330 0 0, clip,height=2.8in]{fig/mobile3.pdf}
%         \label{fig:mlperfapp_run}
%         }
%         \hfill
%         \subfloat[Run details]{\includegraphics[trim=0 0 0 330, clip,height=2.8in]{fig/mobile3.pdf}
%         \label{fig:mlperfapp_results}
%         }
%         \hfill
%         \subfloat[Configuration settings]{\includegraphics[trim=00 0 00 0, clip,height=2.8in]{fig/mobile5.pdf}
%         \label{fig:mlperfapp_config}
%         }
%         \caption{MLPerf Mobile app on Android}
%         \label{fig:MLPerf Mobile app on Android.}
% \end{figure*}
